Groot: An Event-graph-based Approach for Root Cause Analysis in Industrial Settings

For large-scale distributed systems, it's crucial to efficiently diagnose the root causes of incidents to maintain high system availability. The recent development of microservice architecture brings three major challenges (i.e., operation, system scale, and monitoring complexities) to root cause analysis (RCA) in industrial settings. To tackle these challenges, in this paper, we present Groot, an event-graph-based approach for RCA. Groot constructs a real-time causality graph based on events that summarize various types of metrics, logs, and activities in the system under analysis. Moreover, to incorporate domain knowledge from site reliability engineering (SRE) engineers, Groot can be customized with user-defined events and domain-specific rules. Currently, Groot supports RCA among 5,000 real production services and is actively used by the SRE teamin a global e-commerce system serving more than 185 million active buyers per year. Over 15 months, we collect a data setcontaining labeled root causes of 952 real production incidents for evaluation. The evaluation results show that Groot is able to achieve 95% top-3 accuracy and 78% top-1 accuracy. To share our experience in deploying and adopting RCA in industrial settings, we conduct survey to show that users of Grootfindit helpful and easy to use. We also share the lessons learnedfrom deploying and adopting Grootto solve RCA problems inproduction environments.

==> ASE2021-Groot-CR (1) 2/approach.tex <==
\section{Approach}
\begin{figure}[t]
\centering
\resizebox{0.48\textwidth}{!}{ 
  \includegraphics[width=\textwidth]{figures/workflow.PNG}
}
  \caption{Workflow of \system}
  \label{fig:workflow}
\end{figure}

Figure ~\ref{fig:workflow} shows the overall workflow of \system. The triggers for using \system are usually alert(s) from automated anomaly detection, or sometimes an SRE engineer's suspicion. There are three major steps: constructing the service  dependency graph, constructing the event causality graph,  and root cause ranking. The outputs are the root causes ranked by the likelihood. To support fast human investigation experience, we build an interactive UI as shown in  Figure~\ref{fig:UI}: the service dependency, events with causal links and additional details such as raw metrics or the developer contact (of a code deployment event) are presented to the user for next steps. As an  offline part of human investigation, we label/collect a data set, perform validation, and summarize the knowledge for further improvement on all incidents on a daily basis. %as validations and heterogeneous graph learning (HGL)~\cite{qiao2020heterogeneous} to synthesize the knowledge from existing cases in order to further improve the system.

\subsection{Constructing Service Dependency Graph}
\label{sec:appgraph}

The construction of the service dependency graph starts with the initial alerted or suspicious service(s), denoted as $I$. For example, in Figure ~\ref{fig:ex1_dep}, $I=\{\textit{Checkout}\}$. $I$ can contain multiple services based on the range of the trigger alerts or suspicions. We maintain domain service lists where domain-level alerts can be triggered because there is no clear service-level indication.

At the back end, \system maintains a global service dependency graph $G_{global}$ via distributed tracing and log analysis. The directed edge from nodes $A$ to $B$ (two services or system components) in the dependency graph indicates a service invocation or other forms of dependency. In Figure~\ref{fig:ex1_dep}, the black arrows indicate such edges. Bi-directional edges and cycles between the services can be possible and exist. In this work, the global dependency graph is updated daily.%by extracting from one day's total site traffic.

The service dependency (sub)graph $G$ is constructed using $G_{global}$ and $I$. An extended service list $L$ is first constructed by traversing each service in $I$ over $G_{global}$ for a radius range $r$. Each service $u \in L$ can be traversed by at least one service $v \in I$ within $r$ steps: $L=\{u|\exists v\in I, \ dist(u,v)\le r\ or\ dist(v,u)\le r\}$. Then, the service dependency subgraph $G$ is constructed by the nodes in $L$ and the edges between them in $G_{global}$. In our current implementation, $r$ is set to $2$, since this dependency graph may be dynamically extended in the next steps based on events' detail for longer issue chains or additional dependencies.

\subsection{Constructing Event Causality Graph}
\label{sec:causality}

In the second step, \system collects all supported events for each service in $G$ and constructs the causal links between events. 

\subsubsection{Collecting Events}

Table~\ref{tab:events} presents some example event types and detection techniques for \system's production implementation. For detection techniques, ``De Facto'' indicates that the event can be directly collected via a specific API or storage. %The detection can be done passively at the back end continuously then store anomaly events in different databases; or done actively by pulling data and run detection on the fly to save compute resources. 
The detection either runs passively in the back end to reduce delay and improve accuracy, or runs actively for only the services within the dependency graph range to save resources. %For example, low-level error signals or logs are detected actively since they are too many to scale. 

There are three major categories of events: performance metrics, status logs, and developer activities:
\begin{itemize}
    \item \emph{Performance metrics} represent an anomaly of monitored time series metrics. For example, high CPU usage indicates that the service is causing high CPU usage on a certain machine. In this category, most events are continuously and passively detected and stored. %For high CPU usage, threshold indicates the event is created when CPU usage is higher than certain predefined value. TPS spike indicates a spike in transaction per second, since TPS is a moving average value, we use some statistical model learned from historical data to detect such events.
    \item \emph{Status logs} are caused by abnormal system status, such as spike of HTTP error code metrics while accessing other services' endpoints. Different types of error metrics are important and supported in \system, including third-party APIs. For example, Bad Host indicates abnormal patterns on some machines running the service, and can be detected by a  clustering-based ML approach.%Markdown indicates that the whole service is down. 
    \item \emph{Developer activities} are the events generated when a certain activity of developers is triggered, such as code deployment and config change.
\end{itemize}

\begin{table}[t]
\centering
\caption{List of example event types used in \system}
\resizebox{0.4\textwidth}{!}{ 
\begin{tabular}{|c|c|c|}
\hline
Type                                & Event Type                  & Detection Technique  \\ \hline
\multirow{6}{*}{Performance Metrics} & High GC (Overhead)      & Rule-based        \\ \cline{2-3} 
                                    & High CPU Usage          & Rule-based        \\ \cline{2-3} 
%                                    & Out of Memory           & Rule-based        \\ \cline{2-3} 
%                                    & LB Connection Stacking  & Statistical Model \\ \cline{2-3} 
                                    & Latency Spike           & Statistical Model \\ \cline{2-3} 
                                    & TPS Spike               & Statistical Model \\ \cline{2-3} 
                                    & Database Anomaly        & ML Model          \\ \cline{2-3} 
                                    & Business Metric Anomaly & ML Model          \\ \hline
\multirow{4}{*}{Status Logs}        & WebAPI Error            & Statistical Model \\ \cline{2-3} 
                                    & Internal Error          & Statistical Model \\ \cline{2-3} 
                                    & ServiceClient Error     & Statistical Model \\ \cline{2-3} 
                                    & Bad Host                & ML Model          \\ \hline %\cline{2-3} 
%                                    & Hystrix Circuit Break   & De Facto          \\ \hline
\multirow{3}{*}{Developer Activities} & Code Deployment         & De Facto          \\ \cline{2-3} 
                                    & Configuration Change    & De Facto          \\ \cline{2-3} 
                                    & Execute URL             & De Facto          \\ \hline
\end{tabular}
}
\label{tab:events}
\end{table}

In Groot, there are more than a dozen event types such as \emph{Latency Spike} as listed in the column 2 of Table~\ref{tab:events}. 
Each event type is characterized by three aspects: $Name$ indicates the name of this event type; $Lookback Period$ %\footnote{In Figure~\ref{fig:ex2_n1}, there are two periods, 1 day indicates the look-back range if the model has already finished deployment, 4 days indicates the range if the model deployment is still ongoing(incremental deployment).} 
indicates the time range to look back (from the time when the use of \system is triggered) for collecting events of this event type;  $PropertyType$ indicates the types of the properties that an event of this event type should hold. 
$PropertType$  is characterized by a vector of pairs, each of which indicates the string type for a property's name and the primitive type for the property's value such as string, integer, and float. 
Formally, an event type is defined as a tuple: 
$ET = <Name, Lookback Period, PropertyType>$ 
where 
$PropertyType = <(string, \textit{type}_1), ..., (string, \textit{type}_{n})>$ ($n$ is the number of properties that an event of this event type holds). 
%

Each event of a certain event type $ET$ is characterized by four aspects:
$\textit{Service}$ indicates the service name that the event belongs to; $\textit{Type}$ indicates $ET$'s $\textit{Name}$;  $\textit{StartTime}$ indicates the time when the event happens; $\textit{Properties}$ indicates the properties that the event  holds.
Formally, an event is defined as a tuple: 
$e = <Service, Type, StartTime, Properties>$ 
where $Properties$ is an instantiation of $ET$'s  $PropertyType$. 


%and each event is defined as $e = \{<\textit{Property}_i, \textit{value}_i>\}$. Each event type serves as a template for the event instantiation. such as a string, an integer, a float or a set of primitive types while $\textit{value}$ is limited to primitive data types. 
%
%Each event is defined as a sequence of property-value pairs where the set size is $n$.

For example, in Figure~\ref{fig:example1}, the generated event for \emph{Latency Spike in DataCenter-A} in \emph{Service-C} would be $<``\textit{Service-C}'', ``\textit{Latency\ Spike}'', \textit{2021/08/01-12:36:04}, <(``\textit{DataCenter}'',``\textit{DC-1}''),  ...>>$. %So for each service in $G$, we detect/collect and filter the events within specified time range of the alert.

\subsubsection{Constructing Causal Link}

After collecting all events on all services in $G$, in this step, causal links between these events are constructed for RCA ranking. The causal links (red arrows) in Figure~\ref{fig:ex1_cas} are such examples. A causal link represents that the source event can possibly be caused by the target event. SRE knowledge is engineered into rules and used to create causal links between the pairs of events. %As shown in Figure~\ref{fig:example2}, there are two categories of rules: basic rules and conditional rules. 

A rule for constructing a causal link is defined as a tuple:  $Rule = <Target\mbox{-}Type,  Source\mbox{-}Events, Target\mbox{-}Events, Direction,\\ Target\mbox{-}Service,  Condition>$  ($Condition$ can be optionally specified). $Target\mbox{-}Type$ indicates the type of the rule, being either $Static$ or $Dynamic$ (explained further later). $Source\mbox{-}Events$ indicates the type of the causal link's source event ($Source\mbox{-}Events$ are listed in the names of the rules shown in Figures~\ref{fig:ex2_n1},~\ref{fig:ex2_n2} and~\ref{fig:dynamic_example}).   $Target\mbox{-}Events$ indicates the type of the causal link's target event. $Direction$ indicates the direction of the casual link between the target event and source event. $Target\mbox{-}Service$ indicates the service that the target event should belong to. Note that $Target\mbox{-}Service$ in $Static$ rules can be  $Self$, which indicates that the target event would be within the same service as the source event, or $Outgoing$/$Incoming$, which indicates that the target event would belong to the downstream/upstream services of the service that the source event belongs to in $G$.

\begin{figure}[t]
\centering
\includegraphics[width=0.56\columnwidth]{figures/example3.png}
\caption{Example of dynamic rule}
\label{fig:dynamic_example}
\end{figure}

There are two categories of special rules. The first category is \emph{dynamic} rules (i.e., rules whose $Target\mbox{-}Type$  is set to $Dynamic$) to support dynamic dependencies. Here $Target\mbox{-}Service$ does not indicate any of the three possible options listed earlier but indicates the name of the target service that \system would need to create. For example, live DB dependencies are not available due to different tech stacks and high volume. In Figure~\ref{fig:dynamic_example}, a DB issue (DB Markdown) is shown in \emph{Service-A}. Based on the listed \emph{dynamic} rule, \system creates a new ``service'' \emph{DB-1} in $G$, a new event ``Issues'' that belongs to \emph{DB-1}, and a causal link between the two events.  In practice, the SRE teams use dynamic rules to cover a lot of third-party services and database issues since the live dependencies are not easy to maintain.  %However through the internal error messages and dynamic rules, \system is still able to handle these dependencies. %we can still support external inferences. 

The second category of special rules is \emph{conditional} rules. \emph{Conditional} rules are used when some prerequisite conditions should be satisfied before a certain causal link is created. In these rules, $Condition$ is specified with a boolean predicate. As shown in Figure~\ref{fig:ex2_n2}, the SRE teams believe \emph{Latency Spike} events from different services are related only when both events happen within the same data center. Based on this observation, \system would first evaluate the predicate in $Condition$ and build only the causal link when the predicate is true. A conditional rule overwrites the basic rule on the same source-target event pair.

When constructing causal links, \system first applies the \emph{dynamic} rules so that dynamic dependencies and events are first created at once. Then for every event in the initial services (denoted as $I$), if the rule conditions are satisfied, one or many causal links are created from this event to other events from the same or upstream/downstream services. When a causal link is created, the step is repeated recursively for the target event (as a new origin) to create new causal links. After no new causal links are created, the construction of the event causality graph is finished.

% When \system constructs the causal links, \system first processes all dynamic rules as they may create new event nodes in the graph. %\system enumerates the dynamic rules on each existing event node and also on the newly added nodes (There could also be rules applicable to the newly added nodes) until no new event nodes can be created. 


%Each rule is defined as a predicate containing both events' property-value pair. If the predicate evaluates to be true between two events, then we would add the edge in the causality graph. For example, in Figure~\ref{fig:example1}, the rule used to establish the edge between \emph{GC overhead in RNO} and \emph{Latency increase in LVS, RNO, SLC} would be like this: Suppose we are now determining whether there should be a link from event $u$ to event $v$, then this rule would be $u.\text{pool} = v.\text{pool}\ and\ u.\text{type} = ``\text{High GC Overhead}"\ and\ v.\text{type} = ``\text{Latency increase}"\ and\ u.\text{center} \cap v.\text{center} \ne \emptyset$ which holds true for these two events. Each causality link is also associated with a weight which represents the likelihood of causality - we set all initial values as $1.0$. Overtime these value are updated by the statistical analysis result of the collected data set.


\subsection{Root Cause Ranking}
Finally, \system ranks and recommends the most probable root causes from the event causality graph. Similar to how search engines infer the importance of pages by page links, we customize the PageRank \cite{manning2010introduction} algorithm to calculate the root cause ranking; the customized algorithm is named as GrootRank. The input is the event causality graph from the previous step. Each edge is associated with a weighted score for weighted propagation. The default value is set as $1$, and is set lower for alerts with high false-positive rates. 

Based on the observation that dangling nodes are more likely to be the root cause, we customize the personalization vector as $P_n = f_n $ or $P_d = 1$, where $P_d$ is the personalization score for dangling nodes, and $P_n$ is for the remaining nodes; and $f_n$ is a value smaller than 1 to enhance the propagation between dangling nodes. In our work, the parameter setting is $f_n = 0.5$, $\alpha = 0.85$, $max_{iter} = 100$ (which are parameters for the PageRank algorithm). Figure \ref{fig:person} illustrates an example. The grey circles are the events collected from three services and one database. The grey arrows are the dependency links and the red ones are the causal links with the weight of $1$. Both of the PageRank and GrootRank algorithms detect $event 5$ (DB issue) as the root cause, which is expected and correct. However, the PageRank algorithm ranks $event 4$ higher than $event 3$. But $event 3$ of $\textit{Service-C}$ is more likely to be the second most possible root cause (besides $event 5$), because the scores on dangling nodes are propagated to all others equally in each iteration. We can see that $event 3$ is correctly ranked as second using the GrootRank algorithm.

The second step of GrootRank is to break the tied results from the previous step. The tied results are due to the fact that the event graph can contain multiple disconnected sub-graphs with the same shape. We design two techniques to untie the ranking: 
\begin{figure}[t]
\centering
  \includegraphics[width=0.8\columnwidth]{figures/personalvector.png}
  \caption{Example of personalization vector customization}
  \label{fig:person}
\end{figure}

\begin{figure}[t]
\centering
  \includegraphics[width=0.8\columnwidth]{figures/accessdistance.png}
  \caption{Example of using access distance to untie the ranking results}
  \label{fig:untie}
\end{figure}
\begin{enumerate}
\item For each joint event, the access distance (sum) is calculated from the initial anomaly service(s) to the service where the event belongs to. If any ``access'' is not reachable, the distance is set as $d_m+1$ where $d_m$ is the maximum possible distance. The one with shorter access distance (sum) would be ranked higher and vice versa. Figure \ref{fig:untie} presents an example, where \emph{Service-A} and \emph{Service-B} are both initial anomaly services. Since \system suspects that $event 2$ is caused by either $event 3$ or $event 1$ with the same weight. The scores of $event 3$ and $event 1$ are tied. Then, $event 3$ has a score of $1$ (i.e., $0+1$) and $event 1$ has a score of 2 (i.e., $0+2$), since it is not reachable by \emph{Service-B}). Therefore, $event 3$ is ranked first and logical. 
\item For the remaining joint results with the same access distances, \system continues to untie by using the historical root cause frequency of the event types under the same trigger conditions (e.g., checkout domain alerts). This frequency information is generated from the manually labeled dataset. A more frequently occurred root cause type is ranked higher.% than the less frequent ones.
\end{enumerate}


\subsection{Rule Customization Management}

While \system users create or update the rules,  there could be overlaps, inconsistencies, or even conflicts being introduced such as the example in Figure~\ref{fig:ex2_n2}. \system uses two graphs to manage the rule relationships and avoid conflicts for users. One graph is to represent the link rules between events in the same service (\emph{Same-Graph}) while the other is to represent links between different services (\emph{Diff-Graph}). The nodes in these two graphs are the event types defined in Section~\ref{sec:causality}. There are three statuses between each (directional) pair of event types: (1) no rule, (2) only basic rule, and (3) conditional rule (since it overwrites the basic rule). In \emph{Same-Graph}, \system does not allow self-loop as it does not build links between an event and itself.
% but it is possible that we build links between different services with the same event type.

When rule change happens, existing rules are enumerated to build edges in \emph{Same-Graph} and \emph{Diff-Graph} based on $Target\mbox{-}Events$ and $Target\mbox{-}Service$. Based on the users' operation of 
% \begin{itemize}
%     \item 
    (1) ``remove a rule'',  \system removes the corresponding edge on the graphs;
    % \item 
    (2) ``add/update a rule'',  \system checks whether there are existing edges between the given event types, and then warns the users for possible overwrites. 
    % The users can also combine the conditional rules.   % while users are adding basic rules between event types if there are existing conditional rules between them.
    If there are no conflicts, \system just adds/updates edges between the event types.
    % \item Add conditional rules. We would first alert the possible overwrite. Then if users are about to add new conditional rules on the top of existing conditional rules, we would ask the users to combine these two conditions to add a new one. We then build or change all corresponding edges to status 3.
% \end{itemize} 

After all changes, \system extracts the rules from the graphs by converting each edge to a single rule. These rules are automatically implemented, and then tested against our labeled data set. The \system users need to review the changes with validation reports before the changes go online.

% Note that currently we don't check the consistencies between dynamic rules as we cannot process the dynamic event types, but this could be solved in the future by using nodes with symbolic values to represent such event types. 

==> ASE2021-Groot-CR (1) 2/discuss.tex <==
\section{Discussion}

In this section, we discuss some future extension or improvements on the system. 

As we discussed in Section~\ref{sec:anomalyrelated}, there are many related works for anomaly detection. Some approaches are using adaptive concept drifting, which can self-adapt to the target event without manual tuning~\cite{ma2018robust}. One major burden in our event construction is that we need to build different detection strategies/algorithms for different events, while some events are still needed to be manually tuned or detected by rules. Auto-ML is yet to come for anomaly detection, and the interpretability of the result is also a big challenge for end-to-end usability. The filter range for some events also needs manual tuning which requires large amount of domain expertise and is not robust. As of now, we are investing self-adaptive approaches and building time series metrics anomaly detection platform to reduce the event on-boarding cost. 

Also, our approach, which requires a fair amount of ``one-time" effort, utilizes rules to build links between events. A lot of the rules have similar patterns. Despite that our users prefer to have their own control, rules can be inferred from historical patterns. A great extension to this work is the use of machine learning or grammar inference techniques~\cite{wu2019reinam} to automatically or semi-automatically infer the rules.

%At last, since the framework is robust and generic to many use cases, we are planning to release it as open-source system so that we can allow different kinds of users to customize the system based on their own dependencies/events/domains. This also gives us the chance to further speculate \system's performance under different customized scenarios. 

==> ASE2021-Groot-CR (1) 2/eval.tex <==
\section{Evaluation}

We evaluate \system in two aspects: (1) \emph{effectiveness (accuracy)}, which assesses how accurate \system is in  detecting and ranking root causes, and (2) \emph{efficiency}, which assesses how long it takes for \system to derive root causes and conduct end-to-end analysis in action. Particularly, we intend to address the following research questions:
    %\item \emph{User Experience}, which represents how two groups of SREs experience while using \system: domain SREs which use \system to find the root cause to investigate and mitigate, infrastructure SREs which maintain \system to facilitate new requirements.


\begin{itemize}
    \item \textbf{RQ1.} What are the accuracy and efficiency of \system when applied on the collected dataset?
    \item \textbf{RQ2.} How does \system compare with baseline approaches in terms of accuracy?
    \item \textbf{RQ3.} What are the accuracy and efficiency of \system in an end-to-end scenario?
\end{itemize}

% RQ1 aims to see if given a clear triggering event, how would \system perform. RQ2 aims to see whether using adaptive event-driven approach has an advantage compared to baseline in this scenario. RQ3 puts \system in the real time end-to-end scenario, evaluates the \system's efficiency as a whole. 
%2) Conduct a user study to figure out whether \system is actually helpful and user-friendly to the end SRE users.

\subsection{Evaluation Setup}
\label{sec:evalset}
%To measure whether \system can deal with the challenges with industrial settings, we evaluate \system in an environment that is able to represent the real-time large scale distributed system that is running in real world
To evaluate \system in a real-world scenario, we deploy and apply \system  in eBay's e-commerce system that serves more than 159 million active buyers. In particular, we apply \system upon a microservice ecosystem that contains over 5,000 services on three data centers. These services are built on different tech stacks with different programming languages, including Java, Python, Node.js, etc. Furthermore, these services interact with each other by using different types of service protocols, including HTTP, gRPC,  and Message Queue. The distributed tracing of the ecosystem generates 147B traces on average per day.% with 2.8T spans~\cite{opentracing}%The most busy services in the system have more than 50,000 TPS (transactions per second) every day. It is both time-consuming and troublesome for site reliability engineers to manually solve different incidents without the support of tools like \system.  
\subsubsection{Data Set}
\label{sec:dataset}
The SRE teams at eBay help collect a labeled data set containing 952 incidents over 15 months (Jan 2020 - Apr 2021). Each incident data contains the input required by \system (e.g., dependency snapshot and events with details) and the root cause manually labeled by the SRE teams. %To create this data set, 
These incidents are grouped into two categories: 
%we evaluate over 1,500 incidents grouped into two categories: %and around ${40\%}$ cases are missing supported events or caused by external issues (e.g, regional network provider failures). These incidents are categorized as:
\begin{itemize}
\item \emph{Business domain incidents.} These incidents are detected mainly due to their business impact. For example, end users encounter failed interactions, and business or customer experience is impacted, similar to the example in  Figure~\ref{fig:example1}. 
\item \emph{Service-based incidents.} These incidents are detected mainly due to their impact on the service level, similar to the example in Figure~\ref{fig:dynamic_example}.
\end{itemize}

An internal incident may get detected early, and then likely get categorized as a service-based incident or even solved directly by owners without records. On the other hand, infrastructure-level issues or issues of external service providers (e.g., checkout and shipping services) may not get detected until business impact is caused. 

There are 782 business domain incidents and 170 service-based incidents in the data set. For each incident, the root cause is manually labeled, validated, and collected by the SRE teams, who handle the site incidents everyday. For a case with multiple interacting causes, only the most actionable/influential event is labelled as the root cause for the case. These actual root causes and incident contexts serve as the ground truth in our evaluation.


%To trigger the root cause analysis, w
%\begin{enumerate}
%\item\textbf{Business Monitoring}: Business metrics alerts are collected from here. There are around 200+ business time series are detected  by  anomaly detection service every minute.
%\item\textbf{Application Monitoring}:Different application alerts including TPS alerts, Error Spiking alerts, Latency alerts are collected from here. There are around several million time series are detected by  anomaly detection service every minute. 
%\item\textbf{Load Balance Monitoring}: VIP connection number spiking alerts are collected from here. There are around 60k time series are detected by  anomaly detection service every 5 secs. 
%\item\textbf{Deployment system}: Deployment events are collected from here.
%\item\textbf{Site Event system}: Application mark down events and DB mark down events  are collected from here. When a micro-service is not able to talk to its downstream service after retries, it will mark down the downstream service and send a service mark down event to site event system.  Similar to this, when a micro-service is not able to talk to Database, it will mark down the Database and send a DB mark down event to site event system.
%\end{enumerate}

%\subsubsection{Root cause distribution of collected cases}

%\begin{figure}[t]
%\centering
%  \includegraphics[width=\columnwidth]{figures/app_rootcause.png}
%  \caption{Ground-truth RCA distribution of Application-based anomalies}
%  \label{fig:app_rootcause}
%\end{figure}
%\begin{figure}[t]
%\centering
%  \includegraphics[width=\columnwidth]{figures/biz_rootcause.png}
%  \caption{Ground-truth RCA distribution of Business domain anomalies}
%  \label{fig:biz_rootcause}
%\end{figure}

%Figure ~\ref{fig:app_rootcause} and Figure ~\ref{fig:biz_rootcause} shows the root cause distribution of application-based and business domain anomalies in the dataset. From these two charts, we can see that distribution among application-based anomalies is quite diverse while in business domain anomalies, more than 70\% of the anomalies are due to third party errors. We think this imbalance of the distribution among two categories are due to the reason that we cannot monitor third party applications like we do on other parts of the system. So that in the well-monitored applications, the anomalies would be detected earlier by the abnormal metrics before resulting in severe business impact.



\subsubsection{\system Setup}

The \system production system is deployed as three microservices and federated in three data centers with nine 8-core CPUs, 20GB RAM pods each on Kubernetes.

% They are hosted by Gunicorn to scale up. Nginx is used as our routing manager to serve static files and reverse proxying to Gunicorn, and Supervisor to watch the Gunicorn servers in the background and start the processes on reboot.

\subsubsection{Baseline Approaches} 
\label{sec:baseline}
In order to compare \system with other related approaches, we design and implement two baseline approaches for the evaluation:  
\begin{itemize}
    \item \emph{Naive Approach.} This approach directly uses the constructed service dependency graph (Section~\ref{sec:appgraph}). The events are assigned a score by the severeness of the associated anomaly. Then a normalized score for each service is calculated summarizing all the events related to the service. Lastly, the PageRank algorithm is used to calculate the root cause ranking. 
    \item \emph{Non-adaptive Approach.} This approach is not context-aware. It replaces all special rules (i.e., conditional and dynamic ones) with their basic rule versions. Its other parts are identical to \system.
\end{itemize}
The non-adaptive approach can be seen as a baseline for reflecting a group of graph-based approaches (e.g.,  CauseInfer~\cite{chen2014causeinfer} and Microscope~\cite{lin2018microscope}). These approaches also specify certain service-level metrics but lack the context-aware capabilities of \system. Because the tools for these approaches are not publicly available, we implement the non-adaptive approach to approximate these approaches.%of existing graph-based approaches.

\subsection{Evaluation Results}

%Under the settings described in Section~\ref{sec:evalset}, we would be able to evaluate the efficiency and effectiveness of \system in real world scenarios. 

\subsubsection{RQ1}

\label{sec:rq1}

\begin{table}[t]
\centering
\caption{Accuracy of RCA by \system and baselines}
\resizebox{0.9\linewidth}{!}{ 
\begin{tabular}{l|r|r|r|r|r|r|}
\cline{2-7}
                                    & \multicolumn{2}{c|}{\system} & \multicolumn{2}{c|}{Naive} & \multicolumn{2}{c|}{Non-adaptive} \\ \cline{2-7} 
                                    & Top 3        & Top 1       & Top 3         & Top 1      & Top 3         & Top 1 \\ \hline
\multicolumn{1}{|c|}{Service-based}    & 92\%         & 74\%         & 25\%          & 16\%   & 84\% & 62\%       \\ \hline
\multicolumn{1}{|c|}{Business domain} & 96\%         & 81\%        & 2\%          & 1\%   & 28\% & 26\%       \\ \hline
\multicolumn{1}{|c|}{Combined} & 95\%         & 78\%        & 6\%          & 3\%   & 38\% & 33\%       \\ \hline
\end{tabular}
}
 \label{tab:accuracy}
  \vspace{-3.0ex} 
\end{table}

%\begin{figure}[t]
%\centering
%  \includegraphics[width=0.5\textwidth]{figures/app_wrongcause.png}
%  \caption{Ground-truth RCA distribution of Application-based anomalies which \system gives incorrect top-1 result}
%  \label{fig:app_wrongcause}
%\end{figure}
%\begin{figure}[t]
%\centering
%  \includegraphics[width=\columnwidth]{figures/biz_wrongcause.png}
%  \caption{Ground-truth RCA distribution of Business domain anomalies which \system gives incorrect top-1 result}
%  \label{fig:biz_wrongcause}
%\end{figure}

Table~\ref{tab:accuracy} shows the results of applying \system on the collected data set. We measure both top-1 and top-3 accuracy. The top-1 and top-3 accuracy is calculated as the percentage of cases where their ground-truth root cause is ranked within top 1 and top 3, respectively, in \system's results. %All joint rankings must be untied first for fairness. 
\system achieves high accuracy on both incident categories. For example, for business domain incidents, \system achieves 96\% top-3 accuracy.

% While after the causal links construction, the average number of services that are potentially targeted as root cause is reduced to 11.2 and 7.3 for service-based and business domain incidents respectively.
The unsuccessful cases that \system ranks the root cause after top 3 are mostly caused by missing event(s). %Therefore the causality graph is short of necessary causal link(s) or the root cause itself. 
More than one-third of these unsuccessful cases have been addressed by adding necessary events and corresponding rules over time. For example, initially, we had only an event type of general error spike, which mixes different categories of errors and thus causes high false-positive rate. We then have designed different event types for each category of the error metrics (including various internal and client API errors). %We include these cases to reflect a fair setting in production. 
In many cases that \system ranks the root cause after top 1, the labeled root cause is just one of the multiple co-existing root causes. But for fairness,  the SRE teams label only a single root cause in each case. According to the feedback from the SRE teams, \system still facilitates the RCA process for these cases.   %the RCA distribution of these incidents is quite different from the overall ground-truth RCA distribution. More specifically, we find that 

%Every second of an incident RCA process is valuable. 
Our results show that the runtime cost of applying \system is relatively low. For a service-based incident, the average runtime cost of \system is 1.06s while the maximum is 1.69s. For a business domain incident, the average runtime cost is 0.98s while the maximum is 1.14s. %We designed every step as lightweight as possible, for providing timely results in action.
%In order to answer RQ1, we take 219 real production incidents in eBay: 90 App-Search and 129 Domain-Search cases. These cases are handled by the site reliability engineering team or the technical duty officers of eBay. The app-search cases are from the production environment where the trigger anomaly was firstly observed at the application level. The domain-search is built for the most critical business domain - checkout flow. The trigger anomaly of domain search are generated by our ML anomaly detection systems which calculated from different business metrics and customer interaction metrics. Every root cause is manually labeled, and also collect application graph and event context for each ticket. 

%The results are present in table \ref{tab:accuracy}: The \system detects and ranked 100\% and 86\% correct root cause as Top Rank or Top 3 for app-search use cases. For Domain-search are 91\% (Top 1) and 87\% (Top 3). Obviously, our approach is significantly better than the baseline approach. Moreover, the validation for the baseline approach is less strict, the detection is at the application level. For \system accuracy we also restrict on providing the correct root cause event (e.g., code deploy).      

\subsubsection{RQ2}

\label{sec:rq2}

We additionally apply the baseline approaches on the  data set. Table~\ref{tab:accuracy} also shows the evaluation results. The results show that the accuracy of \system is substantially higher than that of the baseline approaches. In terms of the top-1 accuracy, \system achieves 78\% compared with 3\% and 33\% of the naive and non-adaptive approaches, respectively.  In terms of the top-3 accuracy, \system achieves 95\% compared with 6\% and 38\% of the naive and non-adaptive approaches, respectively. 
%In general, \system is 75\% and 45\% more, respectively, in the top-1 accuracy compared with the naive and non-adaptive baselines. \system has even larger advantages in the top-3 accuracy, being 89\% and 57\% more, respectively, compared with the two baselines. For example, \system achieves 81\% in the top-1 accuracy compared with 26\% accuracy of the non-adaptive approach for business domain incidents.%, so that SREs can save time from investigating unrelated services or events.

The naive approach performs worst in all settings, because it blindly propagates the score at service levels.
The accuracy of the non-adaptive approach is much worse for business domain incidents. The reason is that for a business domain incident, it often takes a longer propagation path since the incident is triggered by a group of services, and new dynamic dependencies may be introduced during the event collection, causing more inaccuracy for the non-adaptive approach. %As showed in Section~\ref{sec:rq1}, the causality construction helps to locate the root cause more effectively.  
There can be many non-critical or irrelevant error events in an actual production scenario, aka ``soft'' errors. We suspect that these non-critical or irrelevant events may be ranked higher by the non-adaptive approach since they are similar to injected faults and hard to be distinguished from the actual ones. \system uses dynamic and conditional rules to discover the actual causal links, building fewer links related to such non-critical or irrelevant events for leading to higher accuracy.  

\subsubsection{RQ3}

\begin{table}[]
\centering
\caption{Comparison of \system results on the dataset and end-to-end scenario}
\resizebox{0.95\linewidth}{!}{ 
\begin{tabular}{l|r|r|r|r|}
\cline{2-5}
                                             & \multicolumn{2}{c|}{Service-based} & \multicolumn{2}{c|}{Business Domain} \\ \cline{2-5} 
                                             & Dataset          & End-to-End          & Dataset         & End-to-End         \\ \hline
\multicolumn{1}{|l|}{Top-1 Accuracy}         & 74\%             & 73\%                & 81\%            & 73\%               \\ \hline
\multicolumn{1}{|l|}{Top-3 Accuracy}         & 92\%              & 91\%                & 96\%            & 87\%               \\ \hline
\multicolumn{1}{|l|}{Average Runtime Cost} & 1.06s            & 3.16s               & 0.98s           & 2.98s              \\ \hline
\multicolumn{1}{|l|}{Maximum Runtime Cost} & 1.69s            & 4.56s               & 1.14s           & 3.61s              \\ \hline
\end{tabular}
}
\label{tab:compare}
 \vspace{-3.0ex} 
\end{table}

To evaluate \system under an end-to-end scenario, we apply \system  upon actual incidents in action. Table~\ref{tab:compare} shows the results. The accuracy has a decrease of up to 9 percentage points in the end-to-end scenario, with some failures caused by production issues such as missing data and service/storage failures. In addition, the runtime cost is increased by up to nearly 3 seconds due to the time spent on fetching data from different data sources, e.g., querying the events for a certain time period.

%\system is currently deployed in production, and it helps to detect/confirm the root causes and boost the triaging speed in action for many cases by the time we submit this paper. There is one great case to share: around mid July 2020, there was an issue happened in one of core DB which impacted multiple services across multiple data centers. This caused more than 100 events including more than 40 database mark down events, along with many VIP connection number spike alerts, latency alerts, and error spike alerts happened around the same time. \system was successfully analyzing the root cause to be one problematic DB within a few seconds.

%\subsection{Case Study}
%During the time we put \system integrated into the production environment to work in the real time scenario, we found an interesting case that we would like to share. In mid July 2020, there was an issue happened in one of core DB which impacted multiple applications across multiple data centers. This caused more than 100 events including more than 40 database mark down events, along with many VIP connection number spike alerts, latency alerts, and error spike alerts happened around the same time. \system was successfully analyzing the root cause to be one problematic DB within a few seconds. 
%\system is currently deployed in production and being used for site reliability teams. According to engineers monitoring platform architect, \system explores a new approach to analyze the alerts and events in order to improve observability efficiency. 
%Another comment on \system comes from a senior reliability engineer who now uses \system everyday, "\system fasten our site issue triage a lot. For example, in connection stacking cases, \system clearly shows error chain (connection stacking chain) and points to the last unhealthy pool, which greatly saves our time to check logs of every pool on this chain to find out which pool is the next. And thanks to the \system feature that gathering almost all related events, we can identify which pools or events are related to the ongoing site issue instead of checking every dashboard first to collect pools health information first. Every second improving of issue resolving speed saves thousands of dollars."  



==> ASE2021-Groot-CR (1) 2/experience.tex <==
\section{Experience}



\system currently supports daily SRE work. Figure~\ref{fig:UI} shows a live \system's ``bird's eye view'' UI on an actual simple checkout incident. Service $C$ has the root cause ($Error Spike$) and belongs to an external provider. Although the domain service $A$ also carries an error spike and gets impacted, \system correctly ignores the irrelevant deployment event, which has no critical impact. The events on $C$ are virtually created based on the dynamic rule. %, an API error spike of $B$, and a business alert. 
Note that all causal links (yellow) in the UI indicate ``is  cause of'', being the opposite of ``is caused by'' as  described in Section~\ref{sec:causality} to provide more intuitive UI  for users to navigate through. \system visualizes the dependency and event causality graph with extra information such as an error message. The SRE teams can quickly comprehend the incident context and derived root cause to investigate \system further. A mouseover can trigger ``event enrichment'' based on the event type to present details such as raw metrics and other additional information.%, or links to other tools.
\begin{figure}[t]
\centering
  \includegraphics[width=0.88\linewidth]{figures/GrootUI.png}
  \caption{\system UI in production}
  \label{fig:UI}
   \vspace{-3.0ex} 
\end{figure}





We next share two major kinds of experience:
%In addition, when mouse over any event, the support data pops out such as error message, figures of time series metrics, or contacts of developer activities. 
\begin{itemize}
   \item \textbf{Feedback from \system users and developers},  reflecting the general experience of two groups: (1) domain SRE teams who use \system to find the root cause, and 
% to investigate and mitigate; 
    (2) a centered SRE team who maintains \system to facilitate new requirements. 
%   \system is designed to be SRE-centric, and directly addressing the requirements of both centered and domain SRE teams is important. 
   \item \textbf{Lessons learned}, representing the lessons learned from deploying and adopting \system in production for the real-world RCA process.
\end{itemize}

\subsection{Feedback from \system Users and Developers}

We invite the SRE members who use \system for RCA in their daily work to the user survey. We call them users in this section. We also invite different SRE members responsible for maintaining \system to the developer survey. We call them developers in this section. In total, there are 14 users and 6 developers\footnote{The \system researchers and developers who are authors of this paper are excluded.} who respond to the surveys. 
%

For the user survey, we ask 14 users the following 5 questions (Questions 4-5 have the same choices as Question 1):
\begin{itemize}
    \item \textbf{Question 1.} When \system correctly locates the root cause, how does it help with your triaging experience? Answer choices: Helpful(4), Somewhat Helpful(3), Not Helpful(2), Misleading(1).
    \item \textbf{Question 2.} When \system correctly locates the root cause, how does it save/extend your or the team's triaging time? (Detection and remediation time not included) Answer choices: Lots Of Time Saved(4), Some Time Saved(3), No Time Saved(2), Waste Time Instead(1).
    \item \textbf{Question 3.} Based on your estimation, how much triage time \system would save on average when it correctly locates the root cause? (Detection and remediation time  not included) Answer choices: More than 50\%(4), 25-50\%(3), 10-25\%(2), 0-10\%(1), N/A(0).
    \item \textbf{Question 4.} When \system correctly locates the root cause, do you find that the result ``graph'' provided by \system helps you understand how and why the incident happens?
    \item \textbf{Question 5.} When \system does not correctly locate the root cause, does the result ``graph'' make it easier for your investigation of the root cause?
\end{itemize}


\begin{figure}
    \centering
    \begin{subfigure}[t]{0.45\linewidth}
    \begin{tikzpicture}[scale=0.45]
  \begin{axis}
    [
    ytick={1,2,3,4,5},
    yticklabels={Question 5, Question 4, Question 3, Question 2, Question 1},
    xmin=0
    ]
    \addplot+[
    boxplot prepared={
      average=3.43,
      upper quartile=4.0,
      lower quartile=3.0,
      upper whisker=4.0,
      lower whisker=2.0
    },
    ] coordinates {};
    \addplot+[
    boxplot prepared={
      average=3.64,
      upper quartile=4.0,
      lower quartile=3.0,
      upper whisker=4.0,
      lower whisker=3.0
    },
    ] coordinates {};
    \addplot+[
    boxplot prepared={
      average=2.79,
      upper quartile=3.25,
      lower quartile=2.0,
      upper whisker=4.0,
      lower whisker=2.0
    },
    ] coordinates {};
    \addplot+[
    boxplot prepared={
      average=3.71,
      upper quartile=4.0,
      lower quartile=3.0,
      upper whisker=4.0,
      lower whisker=3.0
    },
    ] coordinates {};
    \addplot+[
    boxplot prepared={
      average=3.79,
      upper quartile=4,
      lower quartile=3.75,
      upper whisker=4.0,
      lower whisker=3.0
    },
    ] coordinates {};
  \end{axis}
\end{tikzpicture}
\caption{From 14 \system users}
\label{fig:survey1}
\end{subfigure}
~
\begin{subfigure}[t]{0.45\linewidth}
    \begin{tikzpicture}[scale=0.45]
  \begin{axis}
    [
    ytick={1,2,3,4,5},
    yticklabels={Question 5, Question 4, Question 3, Question 2, Question 1},
    xmin=0
    ]
    \addplot+[
    boxplot prepared={
      average=3.83,
      upper quartile=4,
      lower quartile=3.75,
      upper whisker=4.0,
      lower whisker=3.0
    },
    ] coordinates {};
    \addplot+[
    boxplot prepared={
      average=3.5,
      upper quartile=4.0,
      lower quartile=3.0,
      upper whisker=4.0,
      lower whisker=3.0
    },
    ] coordinates {};
    \addplot+[
    boxplot prepared={
      average=3.67,
      upper quartile=4.0,
      lower quartile=3.0,
      upper whisker=4.0,
      lower whisker=3.0
    },
    ] coordinates {};
    \addplot+[
    boxplot prepared={
      average=3.67,
      upper quartile=4.0,
      lower quartile=3.0,
      upper whisker=4.0,
      lower whisker=3.0
    },
    ] coordinates {};
    \addplot+[
    boxplot prepared={
      average=3.83,
      upper quartile=4,
      lower quartile=3.75,
      upper whisker=4.0,
      lower whisker=3.0
    },
    ] coordinates {};
  \end{axis}
\end{tikzpicture}
\caption{From 6 \system developers}
\label{fig:survey2}
\end{subfigure}
\caption{Survey results}
 \vspace{-3.0ex} 
\end{figure}

Figure~\ref{fig:survey1} shows the results of the user survey. We can see that most users find \system very useful to locate the root cause. The average score for Question 1 is 3.79, and 11 out of 14 participants find \system very helpful. As for Question 3, \system saves the triage time by 25-50\%. Even in cases that \system cannot correctly locate the root cause, it is still helpful to provide information for further investigation with an average score of 3.43 in Question 5.

For the developer survey, we ask the 6 developers the following 5 questions (Questions 2-5 have the same choices as Question 1):
\begin{itemize}
    \item \textbf{Question 1.} Overall, how convenient is it to change and customize events/rules/domains while using  \system? Answer choices: Convenient(4), Somewhat Convenient(3), Not Convenient(2), Difficult(1).
    \item \textbf{Question 2.} How convenient is it to \emph{change/customize event models} while using \system? 
    \item \textbf{Question 3.} How convenient is it to \emph{add new domains} while using \system? 
    \item \textbf{Question 4.} How convenient is it to \emph{change/customize causality rules} while using \system? 
    \item \textbf{Question 5.} How convenient is it to change/customize \system compared to other SRE tools? 
\end{itemize}

Figure~\ref{fig:survey2} shows the results of the developer survey. Overall, most developers find it convenient to make changes on and customize events/rules/domains in \system. %all questions have very positive responses on average. 5 out of 6 participants find it convenient to make changes on events/rules/domains in \system, while one finds it somewhat convenient. 
% (here domain denotes adding services from different function fields). %We see 3 participants find it somehow convenient in rule customization, indicating that we should make the rule customization easier to use.

\subsection{Lessons learned}
In this section, we share the lessons learned in terms of technology transfer and adoption on using \system in production environments.

\emph{Embedded in Practice.} To build a successful RCA tool in practice, it is important to embed the R\&D efforts in the live environment with SRE experts and users. We have a 30-minute routine meeting daily with an SRE team to manually test and review every site incident. In addition, we actively reach out to the end users for feedback. For example, the users found our initial UI hard to understand. Based on their suggestions, we have introduced alert enrichment with the detailed context of most events, raw metrics, and links to other tools for the next steps. We also make the UI interactive and build user guides, training videos, and sections. As a result, \system has become increasingly practical and well adopted in practice. We believe that R\&D work on observability should be incubated and grown within daily SRE environments. It is also vital to bring developers with rich RCA experience into the R\&D team.

\emph{Vertical Enhancements.} High-confidence and automated vertical enhancements can empower great experiences. \system is enhanced and specialized in critical scenarios such as grouped related %connection stacking 
alerts across services or critical business domain issues, and large-scale scenarios such as infrastructure changes or database issues. Furthermore, the end-to-end automation is also built for integration and efficiency with anomaly detection, RCA, and notification. For notification, domain business anomalies and diagnostic results are sent through communication apps (e.g., slack and email) for better reachability and experience. Within 18 months of R\&D, \system now supports 18 business domains and sub-domains of the company. On average, \system UI supports more than 50 active internal users, and the service sends thousands of results every month. Most of these usages are around the vertical enhancements. 

%\emph{Vertical Enhancement}: During the continued improvements and validations, high accuracy and recurrence scenarios were discovered and enhanced. We created high confidence vertical enhancements that boosted the user's trust and adoption rate. One example here is to use \system for grouped similar connection stacking alerts across the applications or critical domain issues. Thanks to the high customizability of \system, we efficiently enhanced the vertical experiences, such as fine-tuning and specialized events. We then created an end-to-end flow that includes detection, RCA, and notification. Lots of essential incidents with complicated context were supported, such as infra change and database issues. Then, overall efficiency is improved through integrations with other critical site tools. We also attach diagnostic results in the communication apps (e.g., slack, email, and ServiceNow) for better visibility and reachability. Within 18 months of R\&D, we have hundreds of users per month access to the application for 18 domains and sub-domains RCA. We believe for any AIOPs product like \system - vertical enhancements which focus on the domain use cases are essential to success. 


\emph{Data and Tool Reliability.} Reliability is critical to \system itself and requires a lot of attention and effort. For example, if a critical event is missing, \system may infer a totally different root cause, which would mislead users. %the whole causality of an incident may be affected. In this case, it is not helpful that the user can assume only the related metrics/status are fine. 
We estimate the alert accuracy 
%($f1$) 
to be greater than 0.6 in order to be useful. Recall is even more important since \system can effectively eliminate false positive alerts based on the casual ranking. Since there are hundreds of different metrics supported in \system, we spend time to ensure a robust back end by adding partial and dynamic retry logic and high-efficiency cache. \system's unsuccessful cases can be caused by imperfect data, flawed algorithms, or simply code defects. To better trace the reason behind each unsuccessful case, we add a tracing component. Every \system request can be traced back to atomic actions such as retrieving data, data cleaning, and anomaly detection via algorithms.

\emph{Trade-off among Models.} The accuracy and scalability trade-off among anomaly detection models should be carefully considered and tested. In general, some algorithms such as deep-learning-based or ensemble models are more adaptive and accurate than typical ones such as traditional ML or statistical models. However, the former requires more computation resources, operational efforts, and additional system complexities such as training or model fine-tuning. Due to the actual complexities and fast-evolving nature of our context, it is not possible to scale each model (e.g., deep-learning-based models), nor have it deeply customized for every metric at every level. Therefore, while selecting models, we must make careful trade-off in aspects such as accuracy, scalability, efficiency, effort, and robustness. In general, we first set different ``acceptance'' levels by analyzing each event's impact and frequency, and then test different models in staging and pick the one that is good enough. For example, a few alerts such as ``high thread usage'' are defined by thresholds and work just fine even without a model. Some alerts such as  ``service client error'' are more stochastic and require coverage on every metric of every service, and thus we select fast and robust statistical models and actively conduct detection on the fly.  %Business and domain anomaly events can trigger our triaging flow and diagnostics automatically. SRE and monitoring teams spend more time for better and accurate results, such as exercising deep learning approaches, manually correlate critical signals and active improvements for the false positives.

\emph{Phased Incorporation of ML.} In the current industrial settings, ML-powered RCA products still require effective knowledge engineering. Due to the higher complexity and lower ``signal to noise ratio'' of real production incidents, many existing approaches cannot be applied in practice. We believe that the knowledge engineering capabilities can facilitate adoption of technologies such as AIOps. Therefore, \system is designed to be highly customizable and easy to infuse SRE knowledge and to achieve high effectiveness and efficiency. Moreover, a multi-scenario RCA tool requires various and interpretable events from different detection strategies. Auto-ML-based anomaly detection or unsupervised RCA for large service ecosystems is not yet ready in such context.
% resulting in that taking a general ML model is currently not practical in industrial settings.
As for the path of supervised learning, the training data is tricky to label and vulnerable to potential cognitive bias. 
% from SRE engineers
Lastly, the end users often require complete understanding to fully adopt new solutions, because there is no guarantee of correctness. Many recent ML algorithms (e.g., ensemble and deep learning) lack interpretability. Via the knowledge engineering and graph capabilities, \system is able to explain diversity and causality between ML-model-driven and other types of events. Moving forward, we are building a white-box deep learning approach with causal graph algorithms where the causal link weights are parameters and derivable. 
%, while some are manually tuned or detected by rules for certainty and interpretability. For root cause analysis in practice, taking diversified predictive ML anomalies as the major inputs into another ML layer for  root cause analysis, seems too ideal and difficult as mentioned in Section~\ref{sec:intro}. Additionally, there is also a ``chicken-and-egg'' issue for the supervised learning path: collecting training datasets first can be risky and is hard to happen in the SRE domain. Via a graph-based approach, \system is able to explain how diversified and low-level ML events and their connectivity. Also, it effectively and efficiently solve most of the challenge. Lastly, we are more ready for other intelligent solutions with the dataset of 1000+ real production incidents for training, and our AIOPs infrastructure.


==> ASE2021-Groot-CR (1) 2/intro.tex <==
\section{Introduction}

\label{sec:intro}
Since the emergence of microservice  architecture~\cite{balalaie2016microservices}, it has been quickly adopted by many large companies such as Amazon, Google, and Microsoft.
Microservice architecture aims to improve the scalability, development agility, and reusability of these companies' business systems.
Despite these undeniable benefits, different levels of components in such a system can go wrong 
due to the fast-evolving and large-scale nature of microservices architecture~\cite{balalaie2016microservices}. 
Even if there are minimal human-induced faults in code, the system might still be at risk due to anomalies in hardware, configurations, etc. 
Therefore, it is critical to detect anomalies and then efficiently analyze the root causes of the associated incidents, subsequently helping the system reliability 
engineering (SRE) team take further actions to bring the system back to normal.
%Large-scale distributed systems are playing increasingly important roles nowadays due to the increase of global inter-connectivity.
%The reliability of large-scale distributed system is a major concern for both developers and users since different levels of components in such system can go wrong which would cause significant consequences. Even if there are minimal human-related faults, the system might still be at risk due to anomalies in hardware, configurations, etc. Therefore, it is critical to detect anomalies and then efficiently analyze the root causes of the associated incidents. Then the system reliability engineers (SREs) can take further actions to bring the system back to normal.

In the process of recovering a system, it is critical to conduct accurate and efficient root cause analysis (RCA)~\cite{sole2017survey}, the second one of a three-step process. In the first step, anomalies are detected with alerting mechanisms~\cite{zhao2020automatically, xu2017lightweight, tang2012optimizing} %For example, when a critical business metric value exceeds a certain threshold (e.g., customers'  checkout failure rate exceeds 0.1\%).
based on monitoring data such as logs~\cite{aguilera2003performance,zawawy2010log,nair2015learning,lu2017log,gan2019seer}, metrics/key performance indicators (KPIs)~\cite{mace2015pivot,xu2018unsupervised,ma2019ms, meng2020localizing, wu2020microrca}, or a combination thereof~\cite{kim2013root,wang2019grano}.  In the second step, when the alerts are triggered, RCA is performed to analyze the root cause of these alerts and additional events, and to propose recovery actions from the associated incident~\cite{baek2017cloudsight,da2016monitoring,aguilera2003performance}. RCA needs to consider multiple possible interpretations of potential causes for the incident, and these different interpretations could lead to different mitigation actions to be performed.  
In the last step, the SRE teams perform those mitigation actions and recover the system. 
%In the process of recovering the system, root cause analysis (RCA) is one of the most important steps among the three stages: Detection, Triage, and Remediation. In the detection stage, a common practice is to let developers monitor data such as logs~\cite{aguilera2003performance,zawawy2010log,nair2015learning,lu2017log,gan2019seer}, metrics/Key Performance Indicators (KPIs)~\cite{mace2015pivot,xu2018unsupervised,ma2019ms, meng2020localizing, wu2020microrca}, or a combination thereof~\cite{kim2013root,wang2019grano}, and then set up alerting mechanisms~\cite{zhao2020automatically, xu2017lightweight, tang2012optimizing}. %For example, when a critical business metric value exceeds a certain threshold (e.g., customers'  checkout failure rate exceeds 0.1\%). 
%When these alerts are triggered, the triage stage starts. The triage stage's goal is to analyze the root cause of these alerts and propose mitigating actions to recover~\cite{baek2017cloudsight,da2016monitoring,aguilera2003performance}. At last, the remediation stage comes to perform those mitigating actions and resolves the system incident. RCA happens in the triage stage. Multiple possible interpretations of potential causes for the incident need to be considered in RCA. And these different interpretations could lead to different mitigation actions to be performed. Thus, an accurate and efficient RCA is important~\cite{sole2017survey}.

%As the most complex and time-consuming part of the whole process, root cause analysis (RCA) in the triage stage plays a key role. Both the detection and remediation stages have clear conditions such as abnormal metrics or the feedback of performing mitigating actions, while it is highly likely for the triage stage to face a relatively puzzling situation. Usually multiple possible interpretations of potential causes for the anomalies happen and thus different mitigating actions have to be performed. Therefore, an accurate and efficient RCA framework is crucial for the recovery when anomalies happen. 

Based on our industrial SRE experiences, we find that RCA is difficult in industrial practice due to three complexities, particularly under microservice settings:%~\cite{balalaie2016microservices}:%, which existing approaches~\cite{sole2017survey} cannot handle well:
\begin{itemize}
    \item \textbf{\emph{Operational Complexity}}. For large-scale systems, there are typically centered (aka infrastructure) SRE and domain (aka embedded) SRE engineers~\cite{GoogleSRE}. Their communication is often ineffective or limited under the microservice scenarios due to a more diversified tech stack, granular services, and shorter life cycles than traditional systems. The knowledge gap between the centered SRE team and the domain SRE team gets further enlarged and makes RCA much more challenging. Centered SRE engineers have to learn from domain SRE engineers on how the new domain changes work to update the centralized RCA tools. Thus, adaptive and customizable RCA is required instead of one-size-fits-all solutions. %For example, microservice  architecture can involve more diversified tech stacks with shorter life cycles than a traditional system, resulting in larger knowledge gaps since experience on existing tech stack may not mitigate to the new one. Therefore, modern RCA systems must have better adaptability and customizability. However, none of existing approaches~\cite{sole2017survey} provide an easy way to achieve this purpose. 
        
    \item \textbf{\emph{Scale Complexity}}. There could be thousands of services simultaneously running in a large microservice system, resulting in a very high number of monitoring signals. A real incident could cause numerous alerts to be triggered across services. The inter-dependencies and incident triaging between the services are proportionally more complicated than a traditional system~\cite{wu2020microrca}. To detect root causes that may be distributed and many steps away from an initially observed anomalous service, the RCA approach must be scalable and very efficient to digest high volume signals. %Due to the enlarged graph size and complicated dependencies, a lot of existing graph-based approaches tend to construct the causality graph based on static information such as call graph~\cite{meng2020localizing, kim2013root}, which may cause inaccuracy against the complicated dependencies in such scenario.
    
    \item \textbf{\emph{Monitoring Complexity}}. A high quantity of observability data types (metrics, logs, and activities) need to be monitored, stored, and processed, such as intra-service and inter-service metrics. Different services in a system may produce different types of logs or metrics with different patterns. There are also various kinds of activities, such as code deployment or configuration changes. The RCA tools must be able to consume such highly diversified and unstructured data and make inferences. %When we build RCA system in practice, these types are hard to be managed and consumed structurally and effectively. 
    %On the other hand, approaches based on logs analysis would be hard to apply to new tech stack due to the frequent production of different log types. Especially those approaches~\cite{gan2019seer, nair2015learning} that involve learning algorithms may require extra time or larger training data set to deal with the new data type, which would be a burden for a real-time system.


    %\item \textbf{Agile Development with Heterogeneous technology stacks} Microservices architecture allows developers to adapt new technologies to boost productivity and performance, but it also increases the number of different tech stacks involved in the system which requires root cause analysis system to be more flexible. Detecting root causes that are distributed in a domain, or many steps away from an initial-observed anomaly service is harder than ever. This is because of the dynamic services and their dependencies under agile development, as well as the domain knowledge gap from many different decoupled services owners.


\end{itemize}


% The existing approaches~\cite{sole2017survey,meng2020localizing, kim2013root} have limited effectiveness in industrial settings due to the aforementioned complexities,
% and the existing work lacks reports of industrial RCA experiences (as shown in Section~\ref{sec:related}).
% (1) In terms of the operational complexity, few existing approaches~\cite{nguyen2013fchain,chen2014causeinfer,brandon2020graph} have good adaptability toward diversified tech stacks and customizability for different domain contexts and requirements.
% (2) In terms of the scale complexity, most of the related work~\cite{nguyen2013fchain,chen2014causeinfer,weng2018root,qiu2020causality} is evaluated in only a small-scale setting with a few services and without real incidents. For real large-scale system incidents, the inter-dependencies become much more complicated. RCA needs to be event-driven and context-aware, yet not supported by existing graph-based 
% approaches ~\cite{meng2020localizing, kim2013root}, due to the use of static call graphs.
% %  In addition, as the scale goes up, the dependencies among different services or other components in the system also get more complicated. For example, existing graph-based approaches typically construct a causality graph based on static information such as a call  graph~\cite{meng2020localizing, kim2013root}, which may suffer from inaccuracy against the complicated dependencies in industrial settings.
% (3) In terms of the monitoring complexity, existing approaches~\cite{aguilera2003performance,zawawy2010log,nair2015learning,lu2017log,gan2019seer} based on log analysis may not be adaptable to frequent context changes caused by fast-evolving tech stacks, such as different log data types. Especially those approaches~\cite{gan2019seer, nair2015learning} that involve learning algorithms may suffer from severe model drift or scalability issues, imposing runtime-overhead burden for a real-time system. (4) None of the existing work~\cite{sole2017survey} reports industrial RCA experiences, despite the high importance of RCA technology transfer and adoption. 
%These approaches usually capture information about the state of the system by instrumentation~\cite{aguilera2003performance, mace2015pivot, gan2019seer} or monitoring metrics~\cite{mace2015pivot,xu2018unsupervised,ma2019ms, meng2020localizing, wu2020microrca}. Then with techniques such as machine learning~\cite{nair2015learning,gan2019seer,xu2018unsupervised} or heuristics~\cite{wu2020microrca,brandon2020graph,meng2020localizing}, these approaches abstract the RCA problem into logical  constraints~\cite{zawawy2010log, mace2015pivot} or a dependency/causality graph~\cite{brandon2020graph, wu2020microrca, chen2014causeinfer, gan2019seer, schoenfisch2018root, aguilera2003performance, ma2019ms}. Graph models are popular since they can represent the dependencies/causalities between different components in a system. Existing work~\cite{aguilera2003performance,brandon2020graph,schoenfisch2018root,marvasti2013anomaly,weng2018root,wu2020microrca} has already attempted approaches based on probabilistic graphical models to describe the states of the system. These approaches often construct a dependency graph to represent the relationship between different services/applications in the system. Then these approaches run different inference algorithms over the graph such as using statistical models~\cite{schoenfisch2018root} or heuristics to calculate similarity scores~\cite{wu2020microrca,brandon2020graph} to calculate the possibility of each node to be the root cause.


%For example, Azure, one of the world's largest cloud service platform, experienced six major outages in June and July 2020~\cite{AzureHistory}. More importantly, these reliability issues are devastating. In March 2017, S3, another one of the largest cloud service platforms, experienced several hours of outage. This outage is estimated to cause more than \$150 million in revenue loss of related US companies~\cite{S3Outage}.

%Given the large impact caused by these anomalies, preventing them from happening would be ideal. However, prevention would be hard, if not impossible. As we can see in Amazon's official report of the preceding incident, the incident was caused by an S3 team member when she incorrectly entered one of the inputs to the commands, being part of a routine operational step~\cite{S3summary}, although Amazon added new safeguards to prevent such incident from happening again. It would be hard to predict similar issues due to hindsight bias as there could always be situations that are not considered by the developers in system design. Thus, it is important to efficiently detect and diagnose the anomalies and further take actions to bring the system back to normal.

%Moreover, as microservices aim to provide agility in software development~\cite{balalaie2016microservices,larrucea2018microservices}, new tech stack or infrastructure is introduced in the system frequently. In such scenario, experience on existing tech stack may or may not mitigate to the new one. SREs who use the RCA system will have to learn from how the new things work and use such domain knowledge to update the RCA system, for example, what metrics should be focused on the services using new tech stacks or what kind of new events can we mine from the logs data. However, none of the existing approaches provide an easy way for SREs to easily plug in their domain knowledge to allow the RCA system adapt to new tech stacks. 

%In the mean time, although quite some models and approaches have been proposed on RCA~\cite{sole2017survey,ma2020diagnosing,schoenfisch2018root,brandon2020graph,yoon2016dbsherlock,jeyakumar2019explainit,jayathilaka2017performance,zhao2020automatically,marvasti2013anomaly,weng2018root}, in large-scale distributed systems, RCA still poses two major challenges:
%\begin{itemize}
    %\item \textbf{The complexity of the architecture and the large scale of the system.} To achieve the availability and scalability to serve a large number of users, a real-world distributed system often contains thousands of different both logical (e.g., service, application\footnote{In microservices, a service represents a basic process that communicates over the Internet, while an application often consists of a set of services. In our paper, we treat service as synonym of application, and they both serve as a basic component in the application that communicates with other services/applications. We use the item \emph{pool} to represent this idea. By this design, our framework can serve both the microservices scenario and traditional cloud platforms.}, etc.) and physical components (e.g., virtual machine, data center etc.)~\cite{wang2019grano}. The system may not be fully accessible for system developers as it may contain external components provided by third-party developers. It would be time consuming and troublesome to find the root cause due to the large scale and complexity.
    %\item \textbf{The diversity of metrics and events.} There are a lot of metrics of different categories monitored in the system, such as performance metrics (latency, CPU usage or transactions per second (TPS), etc.), status metrics or events (the Java exceptions or HTTP errors threw by applications, etc.), and developer activities (code deploy or configuration change). These different metrics may require different detection strategies and could lead to different mitigating actions.
    %\item \textbf{The dynamic events and real-time demands of the system }
%\end{itemize}

To overcome the limited effectiveness of existing approaches~\cite{sole2017survey,nguyen2013fchain,chen2014causeinfer,ma2020diagnosing,schoenfisch2018root,brandon2020graph,yoon2016dbsherlock,jeyakumar2019explainit,jayathilaka2017performance,zhao2020automatically,marvasti2013anomaly,weng2018root,qiu2020causality,meng2020localizing, kim2013root} (as mentioned in Section~\ref{sec:related}) in industrial settings due to the aforementioned complexities, we propose \system, an event-graph-based RCA approach. %To the best of our knowledge, \system is the first RCA approach with the ability to adapt for diversified events, the scalability for real-world settings and the manageability for contextual information.
In particular, \system constructs an event causality graph, whose basic nodes are monitoring events such as performance-metric deviation events, status change events, and developer activity events. These events carry detailed information to enable accurate RCA. The events and the causalities between them are constructed using specified rules and heuristics (reflecting domain knowledge). In contrast to the existing fully learning-based approaches~\cite{gan2019seer, ma2020diagnosing, zhao2020automatically}, \system provides better transparency and interpretability. Such interpretability is critical in our industrial settings because a graph-based approach can offer visualized reasoning with causality links to the root cause and details of every event instead of just listing the results. Besides, our approach can enable effective tracking of cases and targeted detailed improvements, e.g., by enhancing the rules and heuristics used to construct the graph. 

\system has two salient advantages over existing graph-based approaches:
\begin{itemize}
\item \emph{\textbf{Fine granularity}} (events as basic nodes). First, unlike existing graph-based approaches, which directly use services~\cite{brandon2020graph} or hosts (VMs)~\cite{weng2018root} as basic nodes, \system constructs the causality graph by using monitoring events as basic nodes. Graphs based on events from the services can provide more accurate results to address the monitoring complexity. Second, for the scale complexity, \system can dynamically create hidden events or additional dependencies based on the context, such as adding dependencies to the external service providers and their issues. Third, to construct the causality graph, \system takes the detailed contextual information of each event into consideration for analysis with more depth. Doing so also helps \system incorporate SRE insights with the context details of each event to address the operational complexity.
\item \emph {\textbf{High diversity}} (a wide range of event types supported). First, the causality graph in \system supports various event types such as performance metrics, status logs, and developer activities to address the monitoring complexity. This multi-scenario graph schema can directly boost the RCA coverage and precision. For example, \system is able to detect a specific configuration change on a service as the root cause instead of performance anomaly symptoms, thus reducing triaging efforts and time-to-recovery (TTR). Second, \system allows the SRE engineers to introduce different event types that are powered by different detection strategies or from different sources. For the rules that decide causality between events, we design a grammar that allows easy and fast implementations of domain-specific rules, narrowing the knowledge gap of the operational complexity. Third, \system provides a robust and transparent ranking algorithm that can digest diverse events, improve accuracy, and produce results interpretable by visualization. 
%nstead of the commonly used service~\cite{brandon2020graph} or hosts (VM)~\cite{weng2018root} as the basic nodes of the causality graph, \system goes one level deeper and further, by using monitoring events of these system entities as basic nodes to better represent the complicated incident contexts, as well as precise and accurate root cause detection. The reason for using events as nodes is that each service/application could have multiple related events, and constructing edges between events would help the system to be more accurate among the complicated dependencies as some issues would be created via a ``dynamic'' dependency or propagated via a ``conditional'' dependency. Furthermore, when we construct the causality graph, \system uses rule-based strategies to take the detailed context information of each event into consideration when deciding whether to add a certain causality link. We show an example of such rule in Section~\ref{sec:example}. These two techniques help \system generate more accurate graph representation of the system. %Furthermore, our study in Section~\ref{sec:rq2} also shows that the event-level results and visualization has better interpretability for our end users.
%\item \textbf{Adaptive Customization}. To deal with high velocity development in microservice scenarios, our event-driven causality graph allows a wide range of event types including performance metrics, status logs, and developer activities. \system gives the SREs who maintain the RCA system the ability to define and customize the needed event types into the system and thus use different anomaly detection algorithms (e.g., ML, Statistical, Rule-based) and mitigating strategies against different events. For the rules deciding causality between events, we design the grammar that allows the SREs to easily customize domain-specific rules from their expertise. Furthermore, since we are allowing events such as developer activities (code deployment, etc.), our analysis could directly report the root cause to be a certain service developer activity so the developers of that service can quickly take actions. %into the code change causing the anomaly. 
\end{itemize}

To demonstrate the flexibility and effectiveness of \system, we evaluate it on eBay's production system that serves more than \textbf{159} million active users and features more than \textbf{5,000} services deployed over three data centers. %The TPS (transactions per second) of the most busy services in the system is more than 50,000 everyday, and the distributed tracing of the system generates 147B traces with 2.8T spans~\cite{opentracing} on average per day. 
We conduct experiments on a labeled and validated data set to show that \system achieves 95\% top-3 accuracy and 78\% top-1 accuracy for 952 real production incidents collected over 15 months. %\system outperforms two baseline approaches by 0.65/0.72 and 0.24/0.29, respectively.
Furthermore, \system is deployed in production %of a Fortune 500 e-commerce company 
for real-time RCA, and is used daily by both centered and domain SRE teams, with the achievement of 73\% top-1 accuracy in action. 
Finally, the end-to-end execution time of \system for each incident in our experiments is less than 5 seconds, demonstrating the high efficiency of \system.

We report our experiences and lessons learned when using \system to perform RCA in the industrial e-commerce system. We survey among the SRE users and developers of \system, who find \system easy to use and helpful during the triage stage. Meanwhile, the developers also find the \system design to be desirable to make changes and facilitate new requirements. We also share the lessons learned from adopting \system in production for SRE in terms of technology transfer and adoption.

In summary, this paper makes four main contributions:
\begin{itemize}
    \item An event-graph-based approach named \system for root cause analysis tackling challenges in industrial settings.
    \item Implementation of \system in an RCA framework for allowing the SRE teams to instill domain knowledge.
    \item Evaluation performed in eBay's production environment with more than 5,000 services, for demonstrating \system's effectiveness and efficiency.
    \item Experiences and lessons learned when deploying and applying \system in production.
\end{itemize}




==> ASE2021-Groot-CR (1) 2/macro.tex <==
\usepackage{todonotes}
\usepackage{url}
\usepackage{graphicx}
\usepackage{xspace}
\usepackage{tikz,pgfplots}

\usepgfplotslibrary{statistics}


\newcommand{\system}{\textsc{Groot}\xspace}


==> ASE2021-Groot-CR (1) 2/related.tex <==
\section{Related Work}
\label{sec:related}
%The system recovery process contains two major steps: anomaly detection and root cause analysis. In this section, we would briefly introduce anomaly detection approaches and conduct a literature review on the state of art RCA approaches to point out their limitations in industrial settings.

%\subsection{Anomaly Detection}
%\label{sec:anomalyrelated}

\emph{Anomaly Detection.} Anomaly detection aims to detect potential issues in the system. Anomaly detection approaches using time series data can generally be categorized into three types: (1) batch-processing and historical analysis such as  Surus~\cite{nflxsurus}; (2) machine-learning-based, such as Donut~\cite{xu2018unsupervised}; (3) usage of adaptive concept drift, such as StepWise~\cite{ma2018robust}.

%Anomaly detection aims to detect the potential issues in the system. Anomaly detection approaches using time series data can generally be categorized into three types: The first is processing data in batches and performing historical analysis. These kinds of system has been used in industry such as Netflix's Surus~\cite{nflxsurus}. However it lacks the ability to deal with the real-time scenarios. The second type is based on ML, such as Donut proposed by Xu et al~\cite{xu2018unsupervised}. However, the lack of training data taints the performance of such system. The third type is leveraging adaptive concept drift that may not be robust since they only care about local information~\cite{ma2018robust}.

\system currently uses a combination of manually written thresholds, statistical models, and machine learning (ML) algorithms to detect  anomalies. Since our approach is event-driven, as long as fairly accurate alerts are generated, \system is able to incorporate them. 

%\subsection{Root Cause Analysis}

\emph{Root Cause Analysis.} Traditional RCA approaches (e.g., Adtributor~\cite{bhagwan2014adtributor} and HotSpot~\cite{sun2018hotspot}) find the multi-dimensional combination of attribute values that would lead to certain quality of service (QoS) anomalies. These approaches are effective at discrete static data. Once there are continuous data introduced by time series information, these approaches would be much less effective.

To tackle these difficulties, there are two categories of approaches based on ML and graph, respectively. 

\emph{ML-based RCA.} Some ML-based approaches use features such as time series information~\cite{ma2020diagnosing, weng2018root} and features extracted using textual and temporal information~\cite{zhao2020automatically}. Some other approaches~\cite{xu2018unsupervised} conduct deep learning by first constructing the dependency graph of the system and then representing the graph in a neural network. However, these ML-based approaches face the challenge of lacking training data. Gan et al.~\cite{gan2019seer} proposed Seer to make use of historical tracking data. Although Seer also focuses on the microservice scenario, it is designed to detect QoS violations while lacking support for other kinds of errors. There is also an effort to use unsupervised learning such as GAN~\cite{xu2018unsupervised}, but it is generally hard to simulate large, complicated distributed systems to give meaningful data.

\emph{Graph-based RCA.} A recent survey~\cite{sole2017survey} on RCA approaches categorizes more than 20 RCA algorithms by more than 10 theoretical models to represent the relationships between components in a microservice system.  
Nguyen et al.~\cite{nguyen2013fchain} proposed FChain, which introduces time series information into the graph, but they still use server/VM as nodes in the graph. Chen et al.~\cite{chen2014causeinfer}  proposed CauseInfer, which constructs a two-layered hierarchical causality graph. It applies metrics as nodes that indicate service-level dependency. Schoenfisch et al.~\cite{schoenfisch2018root} proposed to use Markov Logic Network to express conditional dependencies in the first-order logic, but still build dependency on the service level. Lin et al.~\cite{lin2018microscope} proposed Microscope, which targets the microservice scenario. It builds the graph only on service-level metrics so it cannot get full use of other information and lacks customization. Brandon et al. ~\cite{brandon2020graph} proposed to build the system graph using metrics, logs, and anomalies, and then use pattern matching against a library to identify the root cause. However, it is difficult to update the system to facilitate the changing requirements. Wu et al.~\cite{wu2020microrca} proposed MicroRCA, which models both services and machines in the graph and tracks the propagation among them. It would be hard to extend the graph from machines to the concept of other resources such as databases in our paper. 

%Pengfei et al proposed CauseInfer~\cite{chen2014causeinfer}, which constructs a two layered hierarchical causality graph. It applies metrics as nodes which advances service-level dependency. However only considering metrics would restrict the system from getting use of other forms of information which is addressed by the event-based model by \system. Schoenfisch et al proposed to use Markov Logic Network to express conditional dependencies in the first order logic~\cite{schoenfisch2018root}. However their approaches still build dependency on service level. Jinjin et al proposed Microscope~\cite{lin2018microscope} which targets microservices scenario. Despite taking in both communicating and non-communicating dependencies into account, it only builds the graph on service-level metrics so that it cannot get full use of other information and also lacks customization. Brandon et al. proposed an approach that builds the system graph using metrics, logs and anomalies and then use pattern matching against a library to identify the root cause. However it's difficult to update the system to facilitate the changing requirements~\cite{brandon2020graph}.  Li et al. proposed MicroRCA~\cite{wu2020microrca} which models both services and machines in the graph and tracks the propagation among them. It achieves higher accuracy than service-only models but it would be hard to extend the graph from machines to the concept of other resources such as DB in our paper.

As mentioned in Section~\ref{sec:intro}, by using the event graph, \system mainly overcomes the limitations of existing graph-based approaches in two aspects: (1) build a more accurate and precise causality graph use the event-graph-based model; (2) allow adaptive customization of link construction rules to incorporate domain knowledge in order to facilitate the rapid requirement changes in the microservice scenario.
%Our approach would fall into the category of probabilistic graphical model, along with a set of other approaches~\cite{brandon2020graph, schoenfisch2018root}. 

Our \system approach uses a customized page rank algorithm in the event ranking, and can also be seen as an unsupervised ML approach. Therefore, \system is complementary to other ML approaches as long as they can accept our event causality graph as a feature.

\begin{table}[]
\centering
\caption{The scale of experiments in existing RCA approaches’ evaluations (QPS: Queries per second)}
\resizebox{0.45\textwidth}{!}{ 
\begin{tabular}{|l|l|l|l|}
\hline
Approach      & Year   & Scale    & Validated on Real Incidents?                             \\ \hline
FChain~\cite{nguyen2013fchain}        & 2013                  & \textless{}= 10 VMs         & No           \\ \hline
CauseInfer~\cite{chen2014causeinfer}    & 2014             & 20 services on 5 servers       & No       \\ \hline
MicroScope~\cite{lin2018microscope}    & 2018                       & 36 services, $\sim$5000 QPS & No          \\ \hline
APG~\cite{weng2018root}           & 2018                  & \textless{}=20 services on 5 VMs   & No   \\ \hline
Seer~\cite{gan2019seer}          & 2019   & \textless{}=50 services on 20 servers & Partially \\ \hline
MicroRCA~\cite{wu2020microrca}      & 2020                        & 13 services, $\sim$600 QPS     & No       \\ \hline
RCA Graph~\cite{brandon2020graph}     & 2020                          & \textless{}=70 services on 8 VMs  & No    \\ \hline
Causality RCA~\cite{qiu2020causality} & 2020                     & \textless{}=20 services        & No       \\ \hline
\end{tabular}
}
\label{tab:related}
\end{table}

%\begin{tabular}{|l|l|l|l|}
%\hline
%Approach      & Year  & Architecture  & Scale                                \\ \hline
%FChain~\cite{nguyen2013fchain}        & 2013 & VM-based model                   & \textless{}= 10 VMs                    \\ \hline
%CauseInfer~\cite{chen2014causeinfer}    & 2014 & VM-based model                   & 20 services on 5 servers              \\ \hline
%MicroScope~\cite{lin2018microscope}    & 2018 & Kubernetes                       & 36 services, $\sim$5000 QPS           \\ \hline
%APG~\cite{weng2018root}           & 2018 & OpenStack                        & \textless{}=20 services on 5 VMs      \\ \hline
%Seer~\cite{gan2019seer}          & 2019 & Various & \textless{}=50 services on 20 servers \\ \hline
%MicroRCA~\cite{wu2020microrca}      & 2020 & Kubernetes                       & 13 services, $\sim$600 QPS            \\ \hline
%RCA Graph~\cite{brandon2020graph}     & 2020 & DC/OS                            & \textless{}=70 services on 8 VMs      \\ \hline
%Causality RCA~\cite{qiu2020causality} & 2020 & Kubernetes                       & \textless{}=20 services               \\ \hline
%\end{tabular}

\emph{Settings and Scale.} The challenges of operational, scale, and monitoring complexities are observed, especially being substantial in the industrial settings. Hence, we believe that the target RCA approach should be validated at the enterprise scale and against actual incidents for effectiveness. %We find Seer~\cite{gan2019seer} can deal with various languages and frameworks. While both FChain~\cite{nguyen2013fchain} and CauseInfer~\cite{chen2014causeinfer} only take VMs as basic nodes without considering services, the other approaches target at specific architecture. 

Table~\ref{tab:related}  lists  the experimental  settings and scale in existing RCA approaches' evaluations.  All the listed existing approaches are evaluated in a relatively small scenario. 
% MicroScope~\cite{lin2018microscope} runs on a system that has relatively ~1/10 QPS of \system's busiest service (5,000 vs 50,000). However its experiment setting only contains 36 services. 
In contrast, our experiments are performed upon a system containing 5,000 production services on hundreds of thousands of VMs. On average, the sub-dependency graph (constructed in Section~\ref{sec:appgraph}) of our service-based data set is already 77.5 services, more than the total number in any of the listed evaluations. Moreover, 7 out of the 8 listed approaches are evaluated under simulative fault injection on top of existing benchmarks such as RUBiS, which cannot represent real-world incidents;  Seer~\cite{gan2019seer}  collects only the real-world results with no validations. Our data set contains 952 actual incidents collected from real-world settings.

==> ASE2021-Groot-CR (1) 2/summary.tex <==
\section{Conclusion}

In this paper, we have presented our work around root cause analysis (RCA) in industrial settings. To tackle three major RCA challenges (complexities of operation, system scale, and monitoring), we have proposed a novel event-graph-based approach named  \system that constructs a real-time causality graph for allowing adaptive customization. 
%instead of a traditional dependency graph between applications, and allows adaptive customizations. 
%We have implemented our approach as an RCA tool named \system. 
\system can handle diversified anomalies and activities from the system under analysis and is extensible to different approaches of anomaly detection or RCA. We have integrated \system into eBay's large-scale distributed system  containing more than \textbf{5,000} microservices. Our evaluation of \system on a data set consisting of 952 real production incidents shows that \system achieves high accuracy and efficiency across different scenarios and also largely outperforms  baseline graph-based approaches. We also share the lessons learned from deploying and adopting \system in production environments.

==> discuss.tex <==
\section{Discussion}

In this section, we discuss some future extension or improvements on the system. 

As we discussed in Section~\ref{sec:anomalyrelated}, there are many related works for anomaly detection. Some approaches are using adaptive concept drifting, which can self-adapt to the target event without manual tuning~\cite{ma2018robust}. One major burden in our event construction is that we need to build different detection strategies/algorithms for different events, while some events are still needed to be manually tuned or detected by rules. Auto-ML is yet to come for anomaly detection, and the interpretability of the result is also a big challenge for end-to-end usability. The filter range for some events also needs manual tuning which requires large amount of domain expertise and is not robust. As of now, we are investing self-adaptive approaches and building time series metrics anomaly detection platform to reduce the event on-boarding cost. 

Also, our approach, which requires a fair amount of ``one-time" effort, utilizes rules to build links between events. A lot of the rules have similar patterns. Despite that our users prefer to have their own control, rules can be inferred from historical patterns. A great extension to this work is the use of machine learning or grammar inference techniques~\cite{wu2019reinam} to automatically or semi-automatically infer the rules.

%At last, since the framework is robust and generic to many use cases, we are planning to release it as open-source system so that we can allow different kinds of users to customize the system based on their own dependencies/events/domains. This also gives us the chance to further speculate \system's performance under different customized scenarios. 
